On Addressing the Limitations of Graph Neural Networks

This report gives a summary of two problems about graph convolutional networks (GCNs): over-smoothing and heterophily challenges, and outlines future directions to explore.

==> tab_baseline_comparison.tex <==
% Table generated by Excel2LaTeX from sheet 'Results'
\begin{table}[htbp]
  \centering
  \small
  \caption{Accuracy (\%) Comparison of Baseline GNNs and MLP }
  %\resizebox{\textwidth}{!}{
  \setlength{\tabcolsep}{3pt}
    \begin{tabular}{c|c|ccc|c}
    \toprule
    \toprule
    \multirow{2}[2]{*}{Datasets\textbackslash{}Models} & \multirow{2}[2]{*}{MLP} & \multirow{2}[2]{*}{GCN} & \multirow{2}[2]{*}{GAT} & \multirow{2}[2]{*}{GraphSAGE} & Baseline \\
          &       &       &       &       &  Average \\
    \midrule
    Cornell & 85.14 & 60.81 & 59.19 & 82.97 & 67.66 \\
    Wisconsin & 87.25 & 63.73 & 60.78 & 87.84 & 70.78 \\
    Texas & 84.59 & 61.62 & 59.73 & 82.43 & 67.93 \\
    Film  & 36.08 & 30.98 & 29.71 & 35.28 & 31.99 \\
    Chameleon & 46.21 & 61.34 & 61.95 & 47.32 & 56.87 \\
    Squirrel & 29.39 & 41.86 & 43.88 & 30.16 & 38.63 \\
    Cora  & 74.81 & 87.32 & 88.07 & 85.98 & 87.12 \\
    Citeseer & 73.45 & 76.70 & 76.42 & 77.07 & 76.73 \\
    Pubmed & 87.86 & 88.24 & 87.81 & 88.59 & 88.21 \\
    DBLP  & 77.39 & 85.87 & 85.67 & 81.19 & 84.24 \\
     Coauthor CS & 93.72 & 93.91 & 93.41 & 94.38 & 93.90 \\
     Coauthor Phy & 95.77 & 96.84 & 96.32 & OOM   & 96.58 \\
     AMZ Comp & 83.89 & 87.03 & 89.44 & 83.70 & 86.72 \\
    AMZ Photo  & 90.87 & 93.61 & 94.12 & 87.97 & 91.90 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    %}
  \label{tab:comparison_baselines_mlp}%
\end{table}%

%\small
%\setlength{\tabcolsep}{3pt}
%\iffalse \caption{Comparison of Baseline GNN Models and MLP}
%\label{tab:comparison_baselines_mlp}%
%\if

==> tab_comparison_sota.tex <==
% Table generated by Excel2LaTeX from sheet 'Fixed Splits'
\begin{table}[htbp]
  \centering
  \caption{Experimental results on fixed splits provided by \cite{pei2020geom}: average test accuracy $\pm$ standard deviation on 9 real-world benchmark datasets. The best results are highlighted. Results of Geom-GCN, H$_2$GCN and GPRGNN are from \cite{pei2020geom,zhu2020beyond,lingam2021simple}; results of FAGCN, ACM-SGC-1, ACM-SGC-2, ACM-GCN, ACMII-GCN are run by ourselves.}
  \setlength{\tabcolsep}{3pt}
   \scalebox{.75}{
    \begin{tabular}{c|cccccccc}
    \toprule
    \toprule
    Datasets/Models & Geom-GCN & H2GCN & GPRGCN & FAGCN & ACM-SGC-1 & ACM-SGC-2 & ACM-GCN & ACMII-GCN \\
    \midrule
    Cornell & 60.54 $\pm$ 3.67 & 82.70 $\pm$ 5.28 & 78.11 $\pm$ 6.55 & 76.76 $\pm$ 5.87 & 82.43 $\pm$ 5.44 & 82.43 $\pm$ 5.44 & 85.14 $\pm$ 6.07 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{85.95 $\pm$ 5.64} \\
    Wisconsin & 64.51 $\pm$ 3.66 & 87.65 $\pm$ 4.98 & 82.55 $\pm$ 6.23 & 79.61 $\pm$ 1.58 & 86.47 $\pm$ 3.77 & 86.47 $\pm$ 3.77 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{88.43 $\pm$ 3.22} & 87.45 $\pm$ 3.74 \\
    Texas & 66.76 $\pm$ 2.72 & 84.86 $\pm$ 7.23 & 81.35 $\pm$ 5.32 & 76.49 $\pm$ 2.87 & 81.89 $\pm$ 4.53 & 81.89 $\pm$ 4.53 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{87.84 $\pm$ 4.4} & 86.76 $\pm$ 4.75 \\
    Film  & 31.59 $\pm$ 1.15 & 35.70 $\pm$ 1.00 & 35.16 $\pm$ 0.9 & 34.82 $\pm$ 1.35 & 35.49 $\pm$ 1.06 & 36.04 $\pm$ 0.83 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{36.28 $\pm$ 1.09} & 36.16 $\pm$ 1.11 \\
    Chameleon & 60.00 $\pm$ 2.81 & 60.11 $\pm$ 2.15 & 62.59 $\pm$ 2.04 & 46.07 $\pm$ 2.11 & 63.99 $\pm$ 1.66 & 59.21 $\pm$ 2.22 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{66.93 $\pm$ 1.85} & 66.91 $\pm$ 2.55 \\
    Squirrel & 38.15 $\pm$ 0.92 & 36.48 $\pm$ 1.86 & 46.31 $\pm$ 2.46 & 30.83 $\pm$ 0.69 & 45.00 $\pm$ 1.4 & 40.02 $\pm$ 0.96 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{54.4 $\pm$ 1.88} & 51.85 $\pm$ 1.38 \\
    Cora  & 85.35 $\pm$ 1.57 & 87.87 $\pm$ 1.20 & 87.95 $\pm$ 1.18 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{88.05 $\pm$ 1.57} & 86.9 $\pm$ 1.38 & 87.69 $\pm$ 1.07 & 87.91 $\pm$ 0.95 & 88.01 $\pm$ 1.08 \\
    Citeseer & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{78.02 $\pm$ 1.15} & 77.11 $\pm$ 1.57 & 77.13 $\pm$ 1.67 & 77.07 $\pm$ 2.05 & 76.73 $\pm$ 1.59 & 76.59 $\pm$ 1.69 & 77.32 $\pm$ 1.7 & 77.15 $\pm$ 1.45 \\
    PubMed & 89.95 $\pm$ 0.47 & 89.49 $\pm$ 0.38 & 87.54 $\pm$ 0.38 & 88.09 $\pm$ 1.38 & 88.49 $\pm$ 0.51 & 89.01 $\pm$ 0.6 & \cellcolor[rgb]{ .816,  .808,  .808}\textbf{90.00 $\pm$ 0.52} & 89.89 $\pm$ 0.43 \\
    \midrule
    Average Rank & 6.11  & 4.22  & 5.11  & 6.44  & 4.89  & 5.11  & 1.56  & 2.22 \\
    \bottomrule
    \bottomrule
    \end{tabular}%
    }
  \label{tab:performance_comparison_fixed_splits}%
\end{table}%


==> tab_fb_results.tex <==
\begin{table*}[htbp]
  \centering
\tiny
  \caption{Supervised Learning of Shallow GNNs}
  \resizebox{\textwidth}{!}{
    \begin{tabular}{c|ccccccccc}
    \toprule
    Models\textbackslash{}Datasets & Cornell & Wisconsin & Texas & Film  & Chameleon & Squirrel & Cora  & Citeseer  & Pubmed  \\
    \midrule
    GraphSAINT & 70.27 & 71.35 & 72.97 & 17.89 & 43.86 & 33.27 & 84.69 & 73.20 & 89.42 \\
    FB-GraphSAINT & 78.38 & 80.00 & 75.68 & 19.08 & 46.05 & 36.06 & 87.50 & 74.76 & 89.88 \\
    \midrule
    GraphSAGE & 54.05 & 66.00 & 56.76 & 14.67 & 40.13 & 24.14 & 80.64 & 72.36 & 85.49 \\
    FBGraphSAGE & 63.14 & 70.00 & 58.05 & 23.27 & 39.74 & 24.60 & 83.70 & 72.58 & 86.31 \\
    \midrule
    GCN   & 52.70 & 45.88 & 52.16 & 26.86 & 28.18 & 23.96 & 85.77 & 73.68 & 88.13 \\
    FB-GCN & 74.57 & 81.37 & 79.19 & \textbf{36.02} & 41.58 & 26.74 & 85.92 & 75.62 & 89.54 \\
    \midrule
    GAT   & 54.32 & 49.41 & 58.38 & 28.45 & 42.93 & 30.03 & 86.37 & 74.32 & 87.62 \\
    FB-GAT & 66.30 & 69.22 & 65.78 & 33.45 & 48.37 & 32.63 & \textbf{87.72} & 76.21 & 88.05 \\
    \midrule
    GEOM-GCN-p & 60.81 & 64.12 & 67.57 & 31.63 & 60.90 & 38.14 & 84.93 & 75.14 & 88.09 \\
    FB-GEOM-GCN-p & 65.16 & 73.51 & 73.20 & 32.89 & 65.90 & \textbf{45.24} & 85.10 & 76.21 & 88.14 \\
    \midrule
    GEOM-GCN-s & 55.68 & 56.67 & 59.73 & 30.30 & 59.96 & 36.24 & 85.27 & 74.71 & 84.75 \\
    FB-GEOM-GCN-s & 56.78 & 65.49 & 62.86 & 32.50 & 65.12 & 43.39 & 85.57 & 75.31 & 85.77 \\
    \midrule
    GEOM-GCN-i & 56.76 & 58.24 & 57.58 & 29.09 & 60.31 & 33.32 & 85.19 & \textbf{77.99} & 90.05 \\
    FB-GEOM-GCN-i & 57.64 & 62.94 & 66.57 & 32.02 & \textbf{65.66} & 44.11 & 85.97 & 77.89 & \textbf{90.13} \\
    \midrule
    H2GCN-1 & 77.29 & 82.93 & 84.59 & 35.65 & 59.30 & 34.39 & 87.00 & 76.10 & 88.47 \\
    FB-H2GCN-1 & \textbf{79.73} & \textbf{83.72} & \textbf{85.24} & 35.68 & 57.89 & 34.30 & 83.32 & 74.89 & 88.48 \\
    \midrule
    H2GCN-2 & 76.21 & 80.97 & 84.05 & 35.26 & 58.79 & 34.50 & 87.68 & 76.76 & 88.34 \\
    FB-H2GCN-2 & 77.00 & 82.31 & 85.11 & 35.87 & 56.60 & 34.12 & 84.35 & 73.61 & 88.50 \\
    \midrule
    Baseline Average & 62.01 & 63.95 & 65.98 & 27.76 & 50.48 & 32.00 & 85.28 & 74.92 & 87.82 \\
    FB-baseline Average & 68.74 & 74.28 & 72.41 & 31.20 & 54.10 & 35.69 & 85.46 & 75.23 & 88.31 \\
    Average Gain & 6.73  & 10.33 & 6.43  & 3.44  & 3.62  & 3.69  & 0.18  & 0.31  & 0.49 \\
    \midrule
    \midrule
    \multicolumn{10}{c}{Deep Multi-scale GNNs} \\
    \midrule
    GCN2-8 & 70.54 & 73.88 & 71.08 & 33.7  & 60.61 & 37.49 & 85.7  & 75.54 & 88.62 \\
    FBGCN2-8 & 75.95 & 82.35 & 74.59 & 35.37 & 60.43 & 39.69 & 86    & 75.51 & 89.97 \\
    \midrule
    GCN2-16 & 74.86 & 74.12 & 69.46 & 33.62 & 55.48 & 35.98 & 87.3  & 76.54 & 88.28 \\
    FBGCN2-16 & \textbf{77.57} & \textbf{82.55} & 77.03 & 35.12 & 56.78 & 39.38 & 87.5  & 76.67 & 89.39 \\
    \midrule
    GCN2-32 & 72.7  & 70.2  & 69.46 & 31.61 & 53.71 & 35.92 & 88.1  & 76.08 & 87.89 \\
    FBGCN2-32 & 72.81 & 78.63 & 80.27 & 32.99 & 54.98 & 36.81 & 88.3  & 76.49 & 89.1 \\
    \midrule
    GCN2-64 & 71.89 & 68.84 & 66.49 & 28.76 & 54.14 & 36.1  & \textbf{88.5} & 77.08 & 89.57 \\
    FBGCN2-64 & 76.49 & 76.27 & 76.22 & 29.57 & 54.39 & 36.79 & 87.9  & 77    & 89.65 \\
    \midrule
    GCN2*-8 & 72.97 & 78.82 & 72.7  & 34.89 & 62.48 & 40.72 & 86.1  & 75.06 & 89.7 \\
    FBGCN2*-8 & 76.76 & 82.94 & 78.11 & \textbf{35.87} & \textbf{65.11} & 41.19 & 86.9  & 76.32 & 90.2 \\
    \midrule
    GCN2*-16 & 76.49 & 81.57 & 75.41 & 34.18 & 58.86 & 39.88 & 87.5  & 75.8  & 86.69 \\
    FBGCN2*-16 & 76.95 & 82.39 & 76.76 & 35.4  & 59.98 & 40.08 & 87.5  & 76.43 & 89.95 \\
    \midrule
    GCN2*-32 & 74.32 & 77.06 & 77.84 & 33.78 & 56.27 & 37.69 & 88.4  & 76.55 & 89.37 \\
    FBGCN2*-32 & 74.51 & 80.78 & \textbf{84.86} & 34.73 & 57.65 & \textbf{41.24} & 88.2  & 76.89 & 89.92 \\
    \midrule
    GCN2*-64 & 72.43 & 73.53 & 75.41 & 32.72 & 53.82 & 36.83 & 88    & \textbf{77.13} & \textbf{90.3} \\
    FBGCN2*-64 & 75.84 & 81.57 & 80.54 & 34.89 & 57.52 & 39.81 & 87.4  & 77.03 & 89.98 \\
    \midrule
    Baseline Average & 73.275 & 74.7525 & 72.23 & 32.91 & 56.92125 & 37.576 & 87.4  & 76.2225 & 88.8025 \\
    FB-baseline Average & 75.86 & 80.935 & 78.55 & 34.24 & 58.355 & 39.374 & 87.5  & 76.5425 & 89.77 \\
    Average Gain & 2.585 & 6.1825 & 6.316 & 1.335 & 1.43375 & 1.7975 & 0.03  & 0.32  & 0.9675 \\
    \bottomrule
    \bottomrule
    \end{tabular}}
  \label{tab:supervised_learning_shallow_gnns}%
\end{table*}%


% \caption{Supervised Learning of Shallow GNNs}
%\multicolumn{10}{p{66em}}{The results are averaged from $10$ independent runs. The (values) represent the difference of performance brought by patching FB.}
% \label{tab:supervised_learning_shallow_gnns}
%\resizebox{\textwidth}{!}
